Nearly Optimal Robust Subspace Tracking

In this work, we study the robust subspace tracking (RST) problem and obtain one of the first two provable guarantees for it. The goal of RST is to track sequentially arriving data vectors that lie in a slowly changing low-dimensional subspace, while being robust to corruption by additive sparse outliers. It can also be interpreted as a dynamic (time-varying) extension of robust PCA (RPCA), with the minor difference that RST also requires a short tracking delay. We develop a recursive projected compressive sensing algorithm that we call Nearly Optimal RST via ReProCS (ReProCS-NORST) because its tracking delay is nearly optimal. We prove that NORST solves both the RST and the dynamic RPCA problems under weakened standard RPCA assumptions, two simple extra assumptions (slow subspace change and most outlier magnitudes lower bounded), and a few minor assumptions. Our guarantee shows that NORST enjoys a near optimal tracking delay of $O(r \log n \log(1/\epsilon))$. Its required delay between subspace change times is the same, and its memory complexity is $n$ times this value. Thus both these are also nearly optimal. Here $n$ is the ambient space dimension, $r$ is the subspaces' dimension, and $\epsilon$ is the tracking accuracy. NORST also has the best outlier tolerance compared with all previous RPCA or RST methods, both theoretically and empirically (including for real videos), without requiring any model on how the outlier support is generated. This is possible because of the extra assumptions it uses.

==> Tex_Commands.tex <==


\setlength{\arraycolsep}{0.03cm}

%\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\seq}[1]{\left<#1\right>}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\essnorm}[1]{\norm{#1}_{\ess}}

%% THEOREM ENVIRON ---------------------------------------------------
%
%%\newtheorem{theorem}{Theorem}
%%\newtheorem{lem}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{fact}[theorem]{Fact}
%\newtheorem{sigmodel}[theorem]{Asssumption}%{Model}%
%%\newtheorem{corollary}[theorem]{Corollary}
%%\newtheorem{definition}[theorem]{Definition}
%%\newtheorem{remark}[theorem]{Remark}
%%\newtheorem{example}[theorem]{Example}
%%\newtheorem{ass}[theorem]{Assumption}
%%\newtheorem{proposition}[theorem]{Proposition}


% THEOREM ENVIRON ---------------------------------------------------

\newtheorem{theorem}{Theorem}
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{sigmodel}[theorem]{Asssumption}%{Model}%
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{ass}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Proposition}

%from zcom.tex %\input{zcom}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\be}{\protect\[}
\newcommand{\ee}{\protect\]}
\newcommand{\bean}{\begin{eqnarray*} }
\newcommand{\eean}{\end{eqnarray*} }
\newcommand{\bea}{\begin{eqnarray} }
\newcommand{\eea}{\end{eqnarray} }
\newcommand{\ba}{\begin{align*} }
\newcommand{\ea}{\end{align*} }

\newcommand{\nn}{\nonumber}
%\newcommand{\ba}{\begin{array} }
%\newcommand{\ea}{\end{array} }
\newcommand{\re}{\mathbb{R}}
\newcommand{\n}{{\cal N}}
\newcommand{\nois}{g}
\newcommand{\epsbnd}{d(\alpha)}
\newcommand{\epsden}{d_{\mathrm{denom}}(\alpha)}




%commands from Dynamic CS and Modified-CS works
\newcommand{\rest}{\mathrm{rest}}
%{{T_\mathrm{rest}}}
\newcommand{\zetahat}{\hat{\zeta}}
%\newcommand{\sm}{\mathrm{small}}
\newcommand{\tDelta}{{\tilde{\Delta}}}
\newcommand{\tDeltae}{{\tilde{\Delta}_e}}
\newcommand{\tT}{{\tilde{T}}}
%\newcommand{\add}{{\cal A}}
%\newcommand{\rem}{{\cal R}}
%\newtheorem{sigmodel}{Signal Model}

\newcommand{\thr}{{\mathrm{thr}}}
\newcommand{\delthr}{{\mathrm{del-thr}}}
\newcommand{\delbound}{{b}}
\newcommand{\err}{{\mathrm{err}}}
\newcommand{\Q}{{\cal Q}}

\newcommand{\CSres}{{\mathrm{CSres}}}
\newcommand{\diff}{{\mathrm{diff}}}
\newcommand{\Aset}{{\cal A}}
\newcommand{\Rset}{{\cal R}}
\newcommand{\Iset}{{\cal I}}
\newcommand{\Dset}{{\cal D}}
\newcommand{\Sset}{{\cal S}}
\newcommand{\Lset}{{\cal L}}
\newcommand{\Nset}{N}  %{{\cal N}}
\newcommand{\Nhat}{\hat{{\cal N}}}
\newcommand{\N}{{{\cal T}}}
%\newcommand{\del}{\text{del}}
%\newcommand{\Span}{\text{range}}
%\newcommand{\Phat}{\hat{P}}
%\newcommand{\that}{\hat{t}}
%\newcommand{\new}{{\text{new}}}
%\newcommand{\old}{{\text{old}}}
\newcommand{\dif}{{\text{dif}}}
%\newcommand{\thresh}{{\text{thresh}}}
%\newcommand{\Shat}{\hat{S}}
%\newcommand{\lhat}{\hat{\ell}}
\newcommand{\xhat}{\bm{\hat{x}}}
%\newcommand{\That}{\hat{\mathcal{T}}}
%\newcommand{\T}{\mathcal{T}}
%\newcommand{\SE}{\text{SE}}
\newcommand{\mat}{\mathrm{mat}}
%\newcommand{\train}{{\text{train}}}  %(recursive projected CS)
%\newcommand{\train}{{\text{0}}}  %(recursive projected CS)


\newcommand{\bl}{\begin{frame}}
\newcommand{\el} {\end{frame}}
\newcommand{\hd}{\frametitle}
%\newcommand{\sd}{\frametitle}
\newcommand{\cred}{\color{red}} % \bf
\newcommand{\cb}{\color{blue}}
\newcommand{\cbl}{\color{black}}
\newcommand{\cg}{\color{DarkGreen}}
\newcommand{\im}{\vspace{1mm} \item}
\newcommand{\vs}{\vspace{2mm}}
\newcommand{\vsl}{\vspace{1mm}}
\newcommand{\vsm}{\vspace{-2mm}}
\newcommand{\svdeq}{\overset{\mathrm{SVD}}=}
\newcommand{\evdeq}{\overset{\mathrm{EVD}}=}
\newcommand{\qreq}{\overset{\mathrm{QR}}=}


\newcommand{\supp}{\text{support}}
\newcommand{\tw}{\tilde{w}}


\renewcommand\thetheorem{\arabic{section}.\arabic{theorem}}

\newcommand{\tmax}{d} %t_{\mathrm{final}}}

%%% ReProCS Commands %%%%%%%%%%
\newcommand{\bbeta}{\beta}%{\tilde\beta}

\newcommand{\wt}{\bm{w}_t}
\newcommand{\mt}{\bm{m}_t}
\newcommand{\xt}{\bm{x}_t}
\newcommand{\x}{\bm{x}}
\newcommand{\xhatt}{\hat{\bm{x}}_t}
\renewcommand{\l}{\bm{\ell}}
\newcommand{\s}{\bm{s}}
\newcommand{\lt}{\bm{\ell}_t}
%\newcommand{\lhat}{\bm{\hat{\ell}}}
\newcommand{\lhat}{\hat{\bm{\ell}}}

\newcommand{\lhatt}{\hat{\l}_t}   %{\bm{y}_t} %{\y_t}
\newcommand{\yt}{\bm{y}_t}
\newcommand{\y}{\bm{y}}
\newcommand{\tty}{\tilde{\bm{y}}}
%\newcommand{\wt}{\bm{w}_t}
\newcommand{\w}{\bm{w}}
\renewcommand{\v}{{\bm{v}}}
\newcommand{\vt}{\bm{v}_t}

\renewcommand{\a}{\bm{a}}
\newcommand{\e}{\bm{e}} %{\bm{w}}  %
\newcommand{\bnu}{{\bm{\nu}}}
\newcommand{\et}{\bm{e}_t}%{\bm{w}_t}%
\newcommand{\Pt}{\bm{P}_t}
\newcommand{\Pj}{\bm{P}_{(j)}}
\newcommand{\Pjm}{\bm{P}_{(j-1)}}
\newcommand{\Pjs}{\bm{P}_{(j),*}}

\newcommand{\ttrain}{t_{\mathrm{train}}}
\newcommand{\rmnew}{\mathrm{new}}
\newcommand{\new}{\mathrm{new}}
\newcommand{\ex}{\mathrm{ex}}

\newcommand{\Pjnew}{\bm{P}_{(j),\mathrm{new}}}
\newcommand{\at}{\bm{a}_t}
\newcommand{\ats}{\bm{a}_{t,*}}
\newcommand{\atnew}{\bm{a}_{t,\mathrm{new}}}
\newcommand{\I}{\bm{I}}
\newcommand{\Lamt}{\bm{\Lambda}_t}
\newcommand{\Lam}{\bm{\Lambda}}
\newcommand{\Lamtnew}{\bm{\Lambda}_{t,\mathrm{new}}}
\newcommand{\Lamtaunew}{\bm{\Lambda}_{\tau,\mathrm{new}}}
\newcommand{\Lamtstar}{\bm{\Lambda}_{t,*}}
\newcommand{\Lamtex}{\bm{\Lambda}_{t}}
%\newcommand{\bm\Sigma}{\bm{\Lambda}_{(j)}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\J}{\mathcal{J}}


\newcommand{\D}{\bm{D}}
\newcommand{\A}{\bm{A}}
\newcommand{\cM}{\hat{\bm{D}}}  % {\mathcal{\bm{M}}}
\newcommand{\cA}{\bm{D}}    %{\mathcal{\bm{A}}}
\newcommand{\cH}{\bm{H}}


\newcommand{\cs}{\text{cs}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\bigo}{\mathcal{O}}
\newcommand{\newset}{\mathrm{new-set}}
\newcommand{\old}{\mathrm{old}}
\newcommand{\Shat}{\hat{\bm{s}}}
\newcommand{\shat}{\hat{\bm{s}}}
\newcommand{\Lhat}{\hat{\bm{L}}}
%\newcommand{\lhat}{\l}

\newcommand{\Ltilde}{\ttilde{\bm{\ell}}}
\newcommand{\Ltil}{\ttilde{\bm{\ell}}}
\renewcommand{\P}{\bm{P}}
\newcommand{\U}{\bm{U}}
\newcommand{\V}{\bm{V}}
\newcommand{\R}{\bm{R}}
\newcommand{\ch}{{\mathrm{ch}}}
\newcommand{\fx}{{\mathrm{fix}}}
\newcommand{\rot}{{\mathrm{add}}} %{{\mathrm{rot}}}

\newcommand{\mG}{{\mathcal{G}}}
\newcommand{\G}{{\bm{G}}}
\newcommand{\Ghat}{\hat{\bm{G}}}


\renewcommand{\b}{\bm{b}}
\newcommand{\Phat}{\hat{\bm{P}}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Span}{\operatorname{span}} %{\operatorname{range}}
\newcommand{\del}{\mathrm{del}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\add}{\mathrm{add}}%{\mathrm{add}}
\newcommand{\basis}{\operatorname{basis}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\calc}{\mathcal{C}}
\newcommand{\full}{\mathrm{full}}
\newcommand{\cov}{\operatorname{Cov}}

\newcommand{\train}{\mathrm{train}}
\newcommand{\thresh}{\lambda_{\mathrm{thresh}}}  %{\mathrm{thresh}}  %{\hat{\lambda}^-}
\newcommand{\bbbetathresh}{\eta} %{\text{add-thresh}}
\newcommand{\That}{\hat{\mathcal{T}}}
\newcommand{\zetasp}{{\zeta_{*}^+}}
%\newcommand{\SE}{\mathrm{SE}}
\newcommand{\SE}{\sin\theta_{\max}}
\newcommand{\egam}{\Gamma^e}
\newcommand{\Ijk}{\mathcal{I}_{k}}
\newcommand{\that}{{\hat{t}}}
\newcommand{\rmend}{\mathrm{end}}
\newcommand{\M}{\bm{M}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\llceil}{\left\lceil}
\newcommand{\rrceil}{\right\rceil}
\newcommand{\llfloor}{\left\lfloor}
\newcommand{\rrfloor}{\right\rfloor}
\newcommand{\uhat}{{\hat{u}}}
%\newcommand{\lammin}{{\hat{\lambda}_{\train}^-}}
\newcommand{\lammin}{{\lambda}^-}
\newcommand{\lamtrain}{{\lambda}^-} %{{\hat{\lambda}_{\train}^-}}
\newcommand{\jhat}{j}%{\hat{\jmath}}

\newcommand{\rrho}{\rho}
%\newcommand{\Ijk}{\mathcal{I}_{k}}
\newcommand{\Ijkt}{\ttilde{\mathcal{I}}_{k}}
\newcommand{\ghatp}{\hat{g}}%{\hat{g}^+}
\newcommand{\calGjk}{\mathcal{G}_{k}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\Lamcl}{\bm{\Lambda}_{(j),\mathrm{cl}}}
\newcommand{\bnut}{{\bnu}_t}
\newcommand{\bmG}{\bm{G}}
%\newcommand{\L}{\bm{L}}
%\newcommand{\S}{\bm{S}}
\newcommand{\X}{\bm{X}}
\newcommand{\Y}{\bm{Y}}
\newcommand{\W}{\bm{W}}
\newcommand{\Z}{\bm{Z}}
\newcommand{\bE}{\bm{E}}
\newcommand{\F}{\bm{F}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bR}{\bm{R}}

\renewcommand{\H}{\bm{H}}


\newcommand{\outfrac}{\small{\text{max-outlier-frac}}}
\newcommand{\outfracrow}{\small{\text{max-outlier-frac-row}}}
\newcommand{\outfraccol}{\small{\text{max-outlier-frac-col}}}


\newcommand\diagmat[2]{\begin{bmatrix} #1 & \bm{0} \\ \bm{0} & #2\end{bmatrix}} %Usage: $\diagmat{a}{b}$
\newcommand{\one}{\bm{1}}
\newcommand{\polylog}{\mathrm{polylog}}

\newcommand{\matr}[2]{ \left[\begin{array}{cc}
     #1 \\
     #2
   \end{array}
  \right]
  }

\newcommand{\ed}{\mathrm{end}}
\newcommand{\termoneone}{{\mathrm{term11}}}
\newcommand{\SVD}{{SVD}}
\newcommand{\B}{\bm{B}}
\newcommand{\bdel}{b_0}%{b_{0,\del}}
\newcommand{\alphadel}{\alpha}%{\alpha_\del}
\renewcommand{\Re}{\mathbb{R}}

\newcommand{\iidsim}{\overset{\mathrm{iid}}{\sim}} 

==> algo-basicreprocspca-icml.tex <==
\begin{algorithm}[ht!]
\caption{\small{Basic-NORST (with $t_j$ known).  The actual algorithm that detects $t_j$ automatically is Algorithm \ref{algo:auto-reprocs-pca} of Supplement.%
\\ Notation: $\hat{\L}_{t; \alpha} := [\lhat_{t-\alpha + 1}, \cdots, \lhatt]$ and $\SVD_r[\M]$ refers to the top of $r$ left singular vectors of the matrix $\M$.
\\ Obtain $\Phat_0$ by $C (\log r)$ iterations of AltProj on $\Y_{[1,t_\train]}$ with $t_\train=C r$ followed by SVD on the output $\Lhat$.
}
}
\label{norst_basic}
\begin{algorithmic}[1]
%\algrenewcommand\algorithmicindent{0.5em}
\STATE \textbf{Input}:   $\yt$,  \textbf{Output}:  $\shatt$, $\lhatt$,  $\Phat_{(t)}$, $\That_t$
%\textbf{Parameters:} $\omega_{supp}$, $K$, $\alpha$, $\xi$, $r$, $t_j$
\STATE \textbf{Parameters:} $K \leftarrow C\log(1/\zz)$, $\alpha \leftarrow C f^2 r \log n$, $\omega_{supp} \leftarrow \xmint/2$, $\xi \leftarrow \xmint/15$,  $r$ %$t_j$
%\STATE
\STATE {\bf Initialize: } $\tildej~\leftarrow~1$, $k~\leftarrow~1$ $\Phat_{t_\train} \leftarrow \hat{\pt}_{0}$ %\leftarrow SVD_r[\Lhat_\init]$
%($\Lhat_\init$: output of AltProj on $\Y_\init:=\Y_{[1,c r]}$)
%\Phat_{t_\train} \leftarrow
\FOR {$t > t_\train$} %\hspace{7cm}\tikzmark{right}
\STATE $\bpsi \leftarrow \bm{I} - \hat{\pt}_{(t-1)}\hat{\pt}_{(t-1)}{}'$;%\tikzmark{top}
\STATE $\tty_t \leftarrow \bpsi \yt$.
%\STATE $\xhat_{t,cs} \leftarrow \text{CoSaMP}\left(\tilde{\yt}, \bpsi; \ s,\ K_{cosamp}\right)$.
\STATE $\xhat_{t,cs} \leftarrow \arg\min_{\tilde{\bm{x}}} \norm{\tilde{\bm{x}}}_1 \ \text{s.t.}\ \norm{\tilde{\bm{y}}_t - \bpsi \tilde{\bm{x}}} \leq \xi$.
\STATE $\That_t \leftarrow \{i:\ |\xhat_{t,cs}| > \omega_{supp} \}$.
\STATE $\xhat_t \leftarrow \I_{\That_t} ( \bpsi_{\That_t}{}' \bpsi_{\That_t} )^{-1} \bpsi_{\That_t}{}'\tty_t$. %\tikzmark{bottom}
\STATE $\hat{\bm{\ell}}_t \leftarrow \yt - \hat{\bm{x}}_t$.% \hspace{6.75cm} \tikzmark{right2}
\IF {$t = t_j + u \alpha$ for $u = 1,\ 2,\ \cdots,K$} % \tikzmark{top2}
%\STATE \Call{Toggle-Phase}{$\Phat_{j-1}$, $\Lhat_{t, \alpha}$, $\lthres$, $t$}
%\EndIf
%\If {$\mathrm{phase} = \mathrm{update}$}
\STATE $\Phat_{j, k} \leftarrow  \SVD_r[\Lhat_{t; \alpha}]$, $\Phat_{(t)} \leftarrow \Phat_{j,k}$, $k \leftarrow k + 1$.
\ELSE
\STATE $\Phat_{(t)} \leftarrow \Phat_{(t-1)}$.
\ENDIF
\IF{$t = t_j + K\alpha$}
%\STATE $\mathrm{phase} \leftarrow \mathrm{detect}$; $\tildej \leftarrow \tildej + 1$;
\STATE $\Phat_{j} \leftarrow \Phat_{(t)}$, $k \leftarrow 1$, $j \leftarrow j+1$
\ENDIF% \tikzmark{bottom2}
\ENDFOR
\end{algorithmic}
%\AddNote{top}{bottom}{right}{Projected-CS.}
%\AddNote{top2}{bottom2}{right2}{Subspace Update.}
\end{algorithm} 

==> compare_table.tex <==
\begin{table*}[t!]
\caption{\small{Comparing RPCA and RST solutions. All algorithms also require left and right incoherence or left incoherence and $\at$'s bounded (which is similar to right incoherence), and hence these are not compared. The incoherence parameter $\mu$ and the condition numbers are treated as constants.
In general $\rmat=rJ$. {\cred \bf Strong or unrealistic assumptions are shown in red.}
PCP(C) \cite{rpca}, mod-PCP \cite{zhan_pcp_jp},  AltProj \cite{robpca_nonconvex}, RPCA-GD \cite{rpca_gd}, NO-RMC \cite{rmc_gd}, orig-ReProCS \cite{rrpcp_isit15,rrpcp_aistats}, s-ReProCS \cite{rrpcp_dynrpca}. %strm-RPCA \cite{streaming_rpca},
}}
%\vspace{-0.1in}
\begin{center}
\renewcommand*{\arraystretch}{1.01}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|l|l|c|}
\hline
Algorithm & Outlier tolerance & Other Assumptions  & Memory, Time, & \# params \\
%\ & \ & \ & Subs chg det delay (Delay) & pars\\
%{\cred \bf strong incoherence,}
%Delay: $O(r^2 \frac{1}{\epsilon^2} \log n  \log \frac{1}{\epsilon} )$
%\hline
\hline
PCP(C)  & $\outfracrow \in O(1)$& {\cred \bf outlier support: unif. random,} & Memory: $O(n \tmax)$   & zero \\
mod-PCP        & $\outfraccol \in O(1) $ &   $\rmat \leq {c\min(n,\tmax)}/{\log^2 n}$     &  Time: $O(n \tmax^2 \frac{1}{\epsilon})$   & \ \\
%         &  \ &  $\rmat \leq \frac{c\min(n,\tmax)}{\log^2 n}$ & Delay: $\infty$   & \ \\
%\hline
\hline
AltProj   & $\outfracrow \in O\left(1/\rmat\right)$ & $\tmax \ge c \rmat $ & Memory: $O(n \tmax)$   & 2 \\
   & $\outfraccol \in O\left( 1/\rmat\right)$      & \    & Time: $O(n \tmax \rmat^2 \log \frac{1}{\epsilon})$   &   \\
% \ & \ & \ &  Delay: $\infty$  &  \ \\
\hline
RPCA-GD  & $\outfracrow \in O(1/\rmat^{1.5})$     &   $\tmax \ge c \rmat$ & Memory: $O(n \tmax)$   & 5 \\
       & $\outfraccol \in O(1/\rmat^{1.5})$ & \ & Time: $O(n \tmax \rmat \log \frac{1}{\epsilon})$   &  \\
% \ & \ & \ &  Delay: $\infty$  &  \ \\
%\hline
\hline
NO-RMC & $\outfracrow \in O\left(1/\rmat\right)$ & {\cred \bf $\mathbf{c_2 n \ge \tmax \ge c n}$}  & Memory: $O(n \tmax)$   & 4 \\
      & $\outfraccol  \in O(1/\rmat)$            &  & Time: $O(n \rmat^3 \log^2 n \log^2 \frac{1}{\epsilon})$   &  \\
% \ & \ & \ &  Delay: $\infty$  &  \ \\
%\hline
\hline
%{ReProCS} &        {$\outfracrow  \in O(1) $} &  outlier mag. lower bounded,      & {Memory: $O(n\rmat \log n \log \frac{1}{\epsilon} )$}  & 4 \\
%(MERoP)  &       {$\outfraccol \in O(1/\rmat) $} &  $\at$'s independent, $\tmax \ge c r \log n \log \frac{1}{\epsilon}$   & {Time: $O(n \rmat^2 \log n \log^2 \frac{1}{\epsilon})$}  &  \\
%(online)         & \ & first $\rmat$ frames: AltProj assu's                                     &   & \ \\
%\hline
\hline
%mod-PCP \cite{zhan_pcp_jp}  & $\outfracrow \in O(1)$ & {\cred \bf outlier support: unif. random,} & Memory: $O(nr \log^2 n)$   &  \\
%                                        & $\outfraccol \in O(1)$ & {\cred \bf slow subspace change (unrealistic),} & Time: $O(n \tmax r \log^2 n \frac{1}{\epsilon} )$   &   \\
%& \ & $\rmat \leq \frac{c\min(n,\tmax)}{\log^2 n}$ & Delay: $\infty$ & \ \\
%\hline
%{streamingRPCA} &         {$\outfracrow  \in O(1/\rmat) $} & {\cred \bf $\rmat=1$}     & {Memory: $O(n \rmat)$}  & 4 \\
%\cite{streaming_rpca}         & {$\outfraccol \in O(1/\rmat) $} &  \   & {Time: $O(n \tmax \rmat \log \frac{1}{\epsilon})$}  & \ \\
%(online) & \ & \ &  Delay: $\infty$  &  \ \\
%\hline
%
{orig-ReProCS} &         {$\outfracrow  \in O(1) $} &  {\cred \bf outlier support: moving object model,}      & {Memory: $O(nr^2/{\epsilon^2} )$}  & 5 \\
dynamic RPCA, &         {$\outfraccol \in O(1/\rmat) $} & {\cred \bf unrealistic subspace change model,}    &  {Time: $O(n \tmax r \log \frac{1}{\epsilon})$ }  & \\
tracking delay &         \ &  {\cred \bf changed eigenvalues small for some time,}    &  \  & \ \\
too large    &         \ & outlier mag. lower bounded,      &  \ & \ \\
        &  & init data: AltProj assu's, &  \  & \ \\
\                           &   & $\at$'s independent, {\cred \bf $\tmax \ge c r^2/{\epsilon^2}$}    &   & \ \\
\hline
{s-ReProCS:} &        {$\outfracrow  \in O(1) $} & {\cred \bf subspace change: only 1 direc at a time},      & {Memory: $O(nr \log n \log \frac{1}{\epsilon} )$}  & 4 \\
solves d-RPCA &       {$\outfraccol \in O(1/r) $} & outlier mag. lower bounded,      & {Time: $O(n \tmax r \log \frac{1}{\epsilon})$}  &  \\
\& RST w/  &  & $\at$'s independent, $\tmax \ge c r \log n  \log \frac{1}{\epsilon}$.                                     &  \ & \ \\
sub-optimal delay                           &   &  init data: AltProj assumptions    & \  & \ \\
\hline
%
{\bf NORST} &        {$\outfracrow  \in O(1) $} & subspace change: none,       & {Memory: $O(nr \log n \log \frac{1}{\epsilon} )$}  & 4 \\
{\bf  (this work):} solves    &       {$\outfraccol \in O(1/r) $} & outlier mag. lower bounded,  & {Time: $O(n \tmax r \log \frac{1}{\epsilon})$}  &  \\
{\bf d-RPCA \& RST w/}                              &       &   $\at$'s independent, $\tmax \ge c r \log n  \log \frac{1}{\epsilon}$,        &  \ & \ \\
{\bf near-optimal delay}            &  & first $C r$ samples: AltProj assumptions    & \  & \ \\
\hline
\end{tabular}
}
\label{compare_assu}
\end{center}
%\vspace{-0.15in}
%\raggedright \small{\emph{Note}: %The table assumes an $n \times \tmax$ data matrix $\Y:=\L+\X$, where $\L$ has rank $\rmat = rJ$ and the outlier matrix $\X$ is sparse with fraction of nonzeros per row being at most $\outfracrow$ and those per column being at most $\outfraccol$. For simplicity, we ignore all dependence on condition numbers.
%%``\# alg pars": number of algo. parameters.
%%``strong incoh.": $\max_{i,j}|(\U \V')_{i,j}|\le \mu \sqrt{\rmat/n \tmax}$ where $\U, \V$ are left and right singular vectors of $\L$.
%}
%% (for video application, this means slow moving and occasionally static foreground objects are also tolerated). The PCP (Candes et al) result, PCP(C), also achieves this however it needs to assume uniformly randomly distributed outlier support.
\end{table*}


==> medrop_app_sims.tex <==
\section{Detailed Experimental Results} \label{sims_detail}
In this section we present a detailed discussion of the models used to generate the synthetic data, and also present the results on videos.
%the results of numerical experiments on some algorithms on simulated data. Particularly we consider two subspace change models and two sparse outlier models. In the subspace change models we consider the model where at two times there are two directions added and rotated with some of the existing directions in the previous subspace. In the other model we consider the GRASTA type model where we assume that all the directions are rotated but in such a way that the subspace error is bounded. IN the sparse outliers, we consider a novel, moving object type model. This is used to generate outliers in such a way that the fraction of outliers per column and the fraction of outliers per row are different. In the other model, we use the random Bernoulli type matrix where each element of a matrix has a small probability to be present as the sparse outlier. We first describe the Signal Models in detail.
%\subsection{Signal Models}

\begin{figure}[ht!]
\centering
\begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=2 by 1,
            %x descriptions at=edge bottom,
            y descriptions at=edge left,
        },
        % load the style created in the preamble
        my stylecompare,
        %ymin=1e-6, ymax=1e1,
        enlargelimits=false,
        width = .5\linewidth,
        height=4cm,
    ]
       \nextgroupplot[
            %my legend style compare,
            my legend style compare,
            legend style={at={(-.19,1.5)}},
            legend columns = 7,
            ymode=log,
            xlabel=$t$,
            %xlabel={\small{$t$}},
            %ylabel={\small{$\log_{10}\left(\frac{\|\lhatt - \lt\|^2}{\|\lt\|^2}\right)$}},
            ylabel={\small{$\SE(\Phat_{(t)}, \P_{(t)})$}},
            %title=(a)
        ]
	        \addplot table[x index = {0}, y index = {1}]{\ltmodata};
	        \addplot table[x index = {0}, y index = {2}]{\ltmodata};
	        \addplot table[x index = {0}, y index = {3}]{\ltmodata};
	        \addplot table[x index = {0}, y index = {4}]{\ltmodata};
	        \addplot table[x index = {0}, y index = {5}]{\ltmodata};
	        \addplot table[x index = {0}, y index = {6}]{\ltmodata};
	        \addplot table[x index = {0}, y index = {7}]{\ltmodata};
	
	               \nextgroupplot[
            ymode=log,
            %xlabel=$t$,
            xlabel={\small{$t$}},
            %ylabel={\small{$\log_{10}\left(\frac{\|\lhatt - \lt\|^2}{\|\lt\|^2}\right)$}},
            %title=(a)
        ]
	        \addplot table[x index = {0}, y index = {1}]{\ltmodatabern};
	        \addplot table[x index = {0}, y index = {2}]{\ltmodatabern};
	        \addplot table[x index = {0}, y index = {3}]{\ltmodatabern};
	        \addplot table[x index = {0}, y index = {4}]{\ltmodatabern};
	        \addplot table[x index = {0}, y index = {5}]{\ltmodatabern};
	        \addplot table[x index = {0}, y index = {6}]{\ltmodatabern};
	        \addplot table[x index = {0}, y index = {7}]{\ltmodatabern};

    \end{groupplot}
\end{tikzpicture}
%\vspace{-0.25in}
\caption{\footnotesize{Left plot illustrates the $\lt$ error for outlier supports generated using Moving Object Model and right plot illustrates the error under the Bernoulli model. The values are plotted every $k\alpha - 1$ time-frames. The time taken per frame in milliseconds (ms) for the Bernoulli model is shown in legend parentheses.
}}
\vspace{-0.1in}
\label{fig:Comparison}
\end{figure}

\subsection{Synthetic Data}
%\subsubsection{Moving Object Model}
%One practical instance where outlier fractions per row can be larger than those per column is in the case of video moving objects that are either occasionally static or slow moving. The outlier support model for our first and second experiments is inspired by this example. It models a 1D video consisting of a person/object of length $s$ pacing up and down in a room with frequent stops. The object is static for $\bbeta$ frames at a time and then moves down. It keeps moving down for a period of $\tau$ frames, after which it turns back up and does the same thing in the other direction. We let $\bbeta =  \lceil c_0 \tau \rceil$ for a $c_0<1$. With this model, for any interval of the form $[(k_1-1)\tau+1, k_2 \tau]$ for $k_1,k_2$ integers, the outlier fraction per row is bounded by $c_0$. For any general interval of length $\alpha \ge \tau$, this fraction is still bounded by $2c_0$. The fraction per column is $s/n$.
%%\newcommand{\Tt}{\mathcal{T}_t}
%
%\begin{sigmodel}\label{mod:moving_object}
%%\emph{Parameters}: $c_0$, $\tau$, $s$. %Consider a time interval of length $2\tau$ . Denote the support of sparse signal at time $t$ by $\mathcal{T}_t$. Define $\bbeta = \lceil c_0 \tau \rceil$. Then, for the first $\tau$ frames denoting downward motion, [Moving object model]
%Let $\bbeta = \lceil c_0 \tau \rceil$. Assume that the $\Tt$ satisfies the following. For the first $\tau$ frames (downward motion),
%\begin{align*}
%\mathcal{T}_t = \begin{cases}
%[1,\ s], &\quad t \in [1, \beta] \\
%[s+1,\ 2s], &\quad t \in [\beta + 1, 2 \beta] \\
%\vdots \\
%[(1/c_0 - 1)s + 1,\ s/c_0], &\quad t \in [\tau - \beta + 1, \tau] \\
%\end{cases}
%\end{align*}
%for the next $\tau$ frames (upward motion),
%\begin{align*}
%\mathcal{T}_t = \begin{cases}
%[(1/c_0 - 1)s + 1,\ s/c_0], &\quad t \in [\tau + 1,\ \tau + \beta] \\
%[(1/c_0 - 2)s + 1,\ (1/c_0 - 1) s], &\quad t \in [\tau + \beta + 1, \tau + 2\beta] \\
%\vdots \\
%[1,\ s], &\quad t \in [2\tau - \beta + 1, 2\tau]. \\
%\end{cases}
%\end{align*}
%Starting at $t=2\tau+1$, the above pattern is repeated every $2\tau$ frames until the end, $t=\tmax$.
%\end{sigmodel}
%%This model is similar to the model assumed for the guarantees in our older works \cite{rrpcp_isit15,rrpcp_aistats}. %Our current guarantee does not need this model.
%The above model is one practically motivated way to simulate data that is not not generated uniformly at random (or as i.i.d. Bernoulli, which is approximately the same as the uniform model for large $n$). It also provides a way to generate data with a different bounds on outlier fractions per row and per column. The maximum outlier fraction per column is $s/n$. For any time interval of length $\alpha \ge \tau$, the outlier fraction per row is bounded by $2c_0$. A snapshot of the above model is shown in Figure \ref{fig:stmatrix}.
%
%\begin{figure}[ht!]
%\begin{center}
%\resizebox{\linewidth}{!}{
%\includegraphics[clip, scale=0.4, trim=3cm 0cm 0cm 0cm]
%{figures/sparse_matrix.eps}
%}
%\end{center}
%\caption{Illustrating the sparse matrix under the moving-object model (Model \ref{mod:moving_object}). For this figure, $t_\train = 200$. The first $t_\train$ frames have fewer outliers than the rest.}
%\label{fig:stmatrix}
%\end{figure}
%
%\subsubsection{Bernoulli Model}
%For this model we assume that every entry of a matrix $\bm{G}$ is chosen independently with a probability $\rho$, i.e., if we let the sampling operator be denoted by $\mathcal{P}_{\Omega}$, so that $\bm{S} = \mathcal{P}_{\Omega}(\bm{G})$
%\begin{align*}
%(\bm{S})_{ij} = \begin{cases}
%\bm{G}_{ij}, &\quad \text{with probability} \quad \rho \\
%0, &\quad \text{with probability} \quad 1 - \rho
%\end{cases}
%\end{align*}
%Under this model, the expected fraction-outliers-per-row and fraction-outliers-per-column is the same and can be verified to be $\rho$.
%%\subsubsection{Givens' Rotation Model}
%%We  assume that the subspace changes every so often and use $t_j$ to denote the $j$-th change time, for $j=1,2,\dots,J$. We let $t_0:=1$ and $t_{J+1}:=\tmax$.
%%Thus,  $\l_t = \P_{(t)} \a_t$ where $\P_{(t)}$ is an $n \times r$ basis matrix with
%%$\P_{(t)} = \P_j$ for $t \in [t_j, t_{j+1})$, $j=0,1,2,\dots, J$.
%%%
%%The basis matrix $\P_j$ changes by adding a new direction from  $\Span(\P_{j-1,\perp})$ to the subspace and ``rotating it in'' with a small angle $\theta_j$ while also deleting one direction. %
%%To be precise, let $\P_{j,\new}$ denote a new direction, i.e., a direction from $\Span(\P_{j-1,\perp})$, let $\P_{j-1,\fx}$ be the basis matrix for the part of $\Span(\P_{j-1})$ that does not change and let $\P_{j-1,\ch}$ denote the direction from $\Span(\P_{j-1})$ that does change. Then,
%%\bea
%%%\P_j = [\underbrace{\P_{j-1,\fx}}_{n \times (r-1)},  \ \underbrace{\P_{j,\rot}}_{n \times 1}], \text{ where } \P_{j,\rot}:=\P_{j-1,\ch} \cos \theta_j - \P_{j,\new} \sin \theta_j,
%%\P_j = [\P_{j-1,\fx},  \ \P_{j,\rot}], \text{ where } \P_{j,\rot}:=\P_{j-1,\ch} \cos \theta_j - \P_{j,\new} \sin \theta_j,
%%\label{ss_ch}
%%\eea
%%$\P_{j-1,\fx} := (\P_{j-1} \R_{j,0}) \I_{[1,r-1]}$ is a basis for the `fixed' part of the previous subspace, $\P_{j-1,\ch} := (\P_{j-1} \R_{j,0}) \I_{r}$ is the changing direction of the previous subspace, and $\R_{j,0}$ is an $r\times r$ rotation matrix that rotates $\P_{j-1}$ so that the direction that ``changes'' appears as the last column of $(\P_{j-1} \R_{j,0})$.
%%\\
%%The direction that gets deleted is $\P_{j,\del}:= \P_{j-1,\ch} \sin \theta_j + \P_{j,\new} \cos \theta_j$.
%%With \eqref{ss_ch},
%%\[
%%%\|(\I - \P_{(t-1)} \P_{(t-1)}{}') \P_{(t)}\| \le \max_j \|(\I - \P_{j-1} \P_{j-1}{}') \P_{j}\| \le \max_j |\sin \theta_j|.
%%\SE(\P_{(t-1)},\P_{(t)}) \le \max_j \SE(\P_{j-1}, \P_{j}) \le \max_j |\sin \theta_j|.
%%\]
%%%\input{subspace_change_fig}

\subsubsection{Full Rotation Model}
We assume that the subspace changes every so often and use $t_j$ to denote the $j$-th change time, for $j=1,2,\dots,J$. We let $t_0:=1$ and $t_{J+1}:=\tmax$.
Thus,  $\l_t = \P_{(t)} \a_t$ where $\P_{(t)}$ is an $n \times r$ basis matrix with
$\P_{(t)} = \P_j$ for $t \in [t_j, t_{j+1})$, $j=0,1,2,\dots, J$.
%
The basis matrix $\P_j$ changes by the action of a rotation matrix on the left of $\P_j$. To be precise, we have
\begin{align*}
\P_j = e^{\delta_j \bm{B}_j} \P_{j-1}
\end{align*}
where $\delta_j$ controls the subspace error and $\bm{B}_j$ is a skew-Hermitian matrix which ensures that $\P_j{}' \P_j = \I_r$. This is the same model used in \cite{grass_undersampled}.
%\subsection{Experiments}
%We evaluate a set of Robust PCA algorithms under all four combinations of the models described in the previous section and illustrate the performance.
All time comparisons are performed on a Desktop Computer with Intel$^{\textsuperscript{\textregistered}}$ Xeon E$3$-$1240$ $8$-core CPU @ $3.50$GHz and $32$GB RAM.

%\subsubsection{Givens' Rotation and Moving Object}
In this section, we used the following parameters. $n = 1000$, $d = 12,000$, $J = 2$, $t_1 = 3000$, $t_2 = 8000$, $r = 30$, $\delta_1 = 0.001$, $\delta_2 = \delta_1$ and the matrices $\bm{B}_{1}$ and $\bm{B}_2$ are generated as $\bm{B}_{1} = (\tilde{\bm{B}}_1 - \tilde{\bm{B}}_1)$ and $\bm{B}_2 = (\tilde{\bm{B}}_2 - \tilde{\bm{B}}_2)$ where the entries of $\tilde{\bm{B}}_1, \tilde{\bm{B}}_2$ are generated independently from a standard normal distribution. We set $\alpha= 300$. This gives us the basis matrices $\bm{P}_{(t)}$ for all $t$. To obtain the low-rank matrix $\bm{L}$ from this we generate the coefficients $\at \in \mathbb{R}^{r_0}$ as independent zero-mean, bounded random variables. They are $(\at)_i \overset{i.i.d}{\sim} unif[-q_i, q_i]$ where $q_i = \sqrt{f} - \sqrt{f}i/2r$ for $i = 1, 2, \cdots, r - 1$ and $q_{r} = 1$. thus the condition number is $f$ and we selected $f=50$. For the sparse supports, we used Model G.24 \cite{rrpcp_dynrpca} which simulates a moving object pacing in the video. The first $t_{\train} = 100$ frames as the training data, where we generated a smaller fraction of outliers with parameters $s/n = 0.01$, $b_0 = 0.01$ and for $t > t_\train$ we used $s/n = 0.05$ and $b_0 = 0.3$. The sparse outlier magnitudes are generated uniformly at random from the interval $[x_{\min}, x_{\max}]$ with $x_{\min} = 10$ and $x_{\max} = 20$.

We initialized the ReProCS and NORST algorithms using AltProj applied to $\Y_{[1,t_\train]}$. For the parameters to AltProj we used used the true value of $r$, $10$ itertations and a threshold of $0.01$. This, and the choice of $\delta_1$ and $\delta_2$ ensure that $\SE(\Phat_\init, \P_0) \approx \SE(\P_1, \P_0) \approx \SE(\P_2, \P_1) \approx 0.01$. The other algorithm parameters are set as mentioned in the theorem, i.e., $K = \lceil \log(c/\varepsilon) \rceil = 8$, $\alpha = C r \log n = 300$, $\omega = x_{\min}/2 = 5$ and $\xi = 7 x_{\min}/15 = 0.67$, $\lthres = 2 \varepsilon^2 \lambda^+ = 7.5 \times 10^{-4}$. For $l_1$ minimization we used the \texttt{YALL-1} toolbox \cite{yall1} and set the tolerance to $10^{-4}$. For the least-squares step we use the Conjugate Gradient Least Squares instead of the well-known ``backslash'' operator in \texttt{MATLAB} since this is a well conditioned problem. For this we set the tolerance as $10^{-10}$ and the number of iterations as $10$. We have not used any non-trivial optimization to speed up our algorithm. We conjecture that the run-time can be further improved by using \texttt{MEX} files for various sub-routines.

\begin{figure}[ht!]
\begin{center}
\resizebox{.7\linewidth}{!}{
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\\    \newline
	\includegraphics[scale=.2]{figures/orig_MR410.jpg}
&
	\includegraphics[scale=.2]{figures/reprocs_pca_bg_curtain_theory10.jpg}
&
	\includegraphics[scale=.2]{figures/ncrpca_BG_MR410.jpg}
&
	\includegraphics[scale=.2]{figures/gd_BG_MR410.jpg}
&
	\includegraphics[scale=.2]{figures/grasta_BG_MR410.jpg}
&
	\includegraphics[scale=.2]{figures/rpca_BG_MR410.jpg}
\\    \newline
	\includegraphics[scale=.2]{figures/orig_MR540.jpg}
&
	\includegraphics[scale=.2]{figures/reprocs_pca_bg_curtain_theory140.jpg}
&
	\includegraphics[scale=.2]{figures/ncrpca_BG_MR540.jpg}
&
	\includegraphics[scale=.2]{figures/gd_BG_MR540.jpg}
&
	\includegraphics[scale=.2]{figures/grasta_BG_MR540.jpg}
&
	\includegraphics[scale=.2]{figures/rpca_BG_MR540.jpg}
\\    \newline
	\includegraphics[scale=.2]{figures/orig_MR1030.jpg}
&
	\includegraphics[scale=.2]{figures/reprocs_pca_bg_curtain_theory630.jpg}
&
	\includegraphics[scale=.2]{figures/ncrpca_BG_MR1030.jpg}
&
	\includegraphics[scale=.2]{figures/gd_BG_MR1030.jpg}
&
	\includegraphics[scale=.2]{figures/grasta_BG_MR1030.jpg}
&
	\includegraphics[scale=.2]{figures/rpca_BG_MR1030.jpg}
\\    \newline
	\subcaptionbox{original\label{1}}{\includegraphics[scale=.2]{figures/orig_MR1160.jpg}}
&
	\subcaptionbox{NORST\label{1}}{\includegraphics[scale=.2]{figures/reprocs_pca_bg_curtain_theory760.jpg}}
&
	\subcaptionbox{AltProj\label{1}}{\includegraphics[scale=.2]{figures/ncrpca_BG_MR1160.jpg}}
&
	\subcaptionbox{RPCA-GD\label{1}}{\includegraphics[scale=.2]{figures/gd_BG_MR1160.jpg}}
&
	\subcaptionbox{GRASTA\label{1}}{\includegraphics[scale=.2]{figures/grasta_BG_MR1160.jpg}}
&
	\subcaptionbox{PCP\label{1}}{\includegraphics[scale=.2]{figures/rpca_BG_MR1160.jpg}}
\end{tabular}
}
\caption{Comparison of visual performance in Foreground Background separation for the MR dataset. The images are shown at $t = t_{\text{train}} + 10, 140, 630, 760$.}
\end{center}
\end{figure}

For the batch methods used in the comparisons -- PCP, AltProj and  RPCA-GD, we implement the algorithms on $\Y_{[1, t]}$ every $t= t_\train + k\alpha - 1$ frames. Further, we set the regularization parameter for PCP $1/\sqrt{n}$ in accordance with \cite{rpca}. The other known parameters, $r$ for Alt-Proj, outlier-fraction for RPCA-GD, are set using the true values. For online methods we implement the algorithms without modifications. The regularization parameter for ORPCA was set as with $\lambda_1 = 1 / \sqrt{n}$ and $\lambda_2 = 1 / \sqrt{d}$ according to \cite{xu_nips2013_1}. Wherever possible we set the tolerance as $10^-6$ and $100$ iterations to match that of our algorithm.

%We show the results in Figure \ref{fig:Comparison}. The results are averaged over $50$ independent trials.
%\subsubsection{Givens' Rotation and Bernoulli}
%In this section, we used the same parameters for the subspace change model as before. For the first $t_\train$ frames we set $\rho = 0.01$ and for the subsequent frames we set $\rho = 0.2$. The sparse outlier magnitude is generated as above.

%The results are shown in figure \ref{fig:Comparison}. The results are averaged over $50$ independent trials.
%\subsubsection{Full Rotation and Moving Object}
%In this section, we used the following parameters. $n = 1000$, $d = 4600$, $J = 2$,  $t_1 = 1000$, $t_2 = 3400$, $\delta_1 = 0.01$, $\delta_2 = 1.5 \delta_1$ and the matrices $\bm{B}_{1}$ and $\bm{B}_2$ are generated using the \texttt{skewdec} command in MATLAB. The coefficients $\at$ are generated as in the Givens' Rotation model. We used the first $t_{\train} = 400$ frames as the training part, where we generated a smaller fraction of outliers with parameters $s/n = 0.01$, $b_0 = 0.01$ and for $t > t_\train$ we used $s/n = 0.05$ and $b_0 = 0.25$. The sparse outlier magnitude is generated as above.

%We show the results in Figure \ref{fig:Comparison}. The results are averaged over $50$ independent trials.
%\subsubsection{Full Rotation and Bernoulli}

For the Bernoulli model we used the same parameters as above for the subspace change while for the sparse outliers we set $\rho = 0.01$ for the first $t_\train$ frames and $\rho = 0.3$ for the subsequent frames. The sparse outlier magnitudes are generated exactly as above.


%\begin{figure}[ht!]
%\begin{center}
%\begin{subfigure}[t]{0.5\textwidth}
%        \includegraphics[scale=0.18]{figures/bern_full.eps}
%        \caption{Bernoulli + Full Rotation}
%    \end{subfigure}%
%    ~
%    \begin{subfigure}[t]{0.5\textwidth}
%        \includegraphics[scale=0.18]{figures/bern_givens.eps}
%        \caption{Bernoulli + Givens' Rotation}
%    \end{subfigure}
%    \begin{subfigure}[t]{0.5\textwidth}
%        \includegraphics[scale=0.18]{figures/MO_full.eps}
%        \caption{Moving Object + Full Rotation}
%    \end{subfigure}%
%    ~
%    \begin{subfigure}[t]{0.5\textwidth}
%        \includegraphics[scale=0.18]{figures/MO_givens.eps}
%        \caption{Moving Object + Givens' Rotation}
%    \end{subfigure}
%\end{center}
%\caption{First row ((a), (b)): Illustrate the $\lt$ error for outlier supports generated using Bernoulli Model. The values are plotted every $k\alpha - 1$ time-frames. The results are averaged over $50$ iterations. Second row ((c), (d)) illustrate the the normalized $\lt$ error using the Moving Object outlier support model. They are plotted every $k\alpha - 1$ time-frames. The plots clearly corroborates the nearly-exponential decay of the subspace error as well as the error in $\lt$. Furthermore observe that MEDRoP is the only algorithm that works under all possible combinations.}
%\label{fig:Comparison}
%\end{figure}
%
%\begin{table}
%\begin{center}
%\caption{\small{Average time taken to process one frame of data (in milliseconds) under the given model.}}
%\resizebox{\linewidth}{!}{
%\begin{tabular}{@{}llllllll@{}}
%\toprule
%Model & GRASTA & ORPCA & ReProCS & MEDRoP & AltProj & RPCA-GD & Offline ReProCS \\ \midrule
%Bern + Full & $\textbf{0.57}$  & $3.3$ & $1.2$ & $1.3$ & $27.2$ & $25.8$& $2.0$ \\
%Bern + Givens' & $\textbf{0.54}$ & $7.1$ & $3.7$ & $3.8$ & $21.9$ & $90.7$& $8.2$ \\
%MO + Full & $\textbf{0.57}$  & $3.3$ & $1.2$ & $1.3$ & $27.2$ & $25.8$& $2.0$ \\
%MO + Givens' & $\textbf{0.56}$  & $3.6$ & $1.3$ & $1.3$ & $37.8$ & $38.0$& $2.6$ \\ \bottomrule
%\end{tabular}
%}
%\end{center}
%\end{table}
%
%We also perform another experiment where instead of using all the frames until the present frame for the batch techniques, we use just the previous alpha frames to get an estimate. Specifically we use the same data as in experiment (b) above. We implement AltProj and PCP in the method described above. Note that even though theoretically using $\alpha$ frames only gives a better fraction of outliers that can be tolerated, since the value of $\alpha$ is very small ($200$) the algorithms fail to  attain the original performance. See Fig. \ref{fig:ComparisonAlpha}
%
%\begin{figure}[ht!]
%\begin{center}
%        \includegraphics[scale=0.18]{figures/bern_givens_alpha.eps}
%        \caption{Bernoulli + Givens' Rotation}
%\end{center}
%\caption{Illustrates the additional experiment to disclaim the theoretical advantage of using just $\alpha$ frames.}
%\label{fig:ComparisonAlpha}
%\end{figure}

\begin{figure}[ht!]
\begin{center}
\resizebox{.75\linewidth}{!}{
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\\    \newline
	\includegraphics[scale=.15]{figures/orig_LB660.jpg}
&
	\includegraphics[scale=.15]{figures/reprocs_pca_bg_LB260.jpg}
&
	\includegraphics[scale=.15]{figures/ncrpca_BG_LB660.jpg}
&
	\includegraphics[scale=.15]{figures/gd_BG_LB660.jpg}
&
	\includegraphics[scale=.15]{figures/grasta_BG_LB660.jpg}
&
	\includegraphics[scale=.15]{figures/rpca_BG_LB660.jpg}
\\    \newline
	\includegraphics[scale=.15]{figures/orig_LB945.jpg}
&
	\includegraphics[scale=.15]{figures/reprocs_pca_bg_LB545.jpg}
&
	\includegraphics[scale=.15]{figures/ncrpca_BG_LB945.jpg}
&
	\includegraphics[scale=.15]{figures/gd_BG_LB945.jpg}
&
	\includegraphics[scale=.15]{figures/grasta_BG_LB945.jpg}
&
	\includegraphics[scale=.15]{figures/rpca_BG_LB945.jpg}
\\    \newline
	\subcaptionbox{original\label{1}}{\includegraphics[scale=.15]{figures/orig_LB1010.jpg}}
&
	\subcaptionbox{NORST\label{1}}{\includegraphics[scale=.15]{figures/reprocs_pca_bg_LB610.jpg}}
&
	\subcaptionbox{AltProj\label{1}}{\includegraphics[scale=.15]{figures/ncrpca_BG_LB1010.jpg}}
&
	\subcaptionbox{RPCA-GD\label{1}}{\includegraphics[scale=.15]{figures/gd_BG_LB1010.jpg}}
&
	\subcaptionbox{GRASTA \label{1}}{\includegraphics[scale=.15]{figures/grasta_BG_LB1010.jpg}}
&
	\subcaptionbox{PCP\label{1}}{\includegraphics[scale=.15]{figures/rpca_BG_LB1010.jpg}}
\end{tabular}
}
\caption{Comparison of visual performance in Foreground Background separation for the Lobby (LB) dataset. The recovered background images are shown at $t = t_\train + 260, 545, 610$.}% The time taken for each of the techniques is shown in parentheses. For MEDRoP the time denotes training-time + test-time.}
\end{center}
\end{figure}

\subsection{Real Video Experiments}
In this section we provide simulation results for on real video, specifically the Meeting Room (MR) sequence. The meeting room sequence is set of $1964$ images of resolution $64 \times 80$. The first $1755$ frames consists of outlier-free data. Henceforth, we consider only the last $1209$ frames. For NORST, we used the first $400$ frames as the training data. In the first $400$ frames, a person wearing a black shirt walks in, writes something on the board and goes back. In the subsequent frames, the person walks in with a white shirt. This is a challenging video sequence because the color of the person and the color of the curtain are hard to distinguish. NORST is able to perform the separation at around $43$ frames per second.

We obtained an estimate using the Alt Proj algorithm. For the Alt Proj algorithm we set $r = 40$. The remaining parameters were used with default setting. For NORST, we set $\alpha = 60$, $K = 3$, $\xi_t = \|\bm{\Psi} \hat{\bm{\ell}}_{t-1}\|_2$. We found that these parameters work for most videos that we verified our algorithm on. For RPCA-GD we set the ``corruption fraction'' $\alpha = 0.2$ as described in the paper. {\em Lobby dataset}: This dataset contains $1555$ images of resolution $128 \times 160$. The first $341$ frames are outlier free. Here we use the first $400$ ``noisy'' frames as training data. The Alt Proj algorithm is used to obtain an initial estimate with rank, $r = 40$. The parameters used in all algorithms are exactly the same as above. NORST achieves a ``test'' processing rate of $16$ frames-per-second. {\em Switch Light dataset}: This dataset contains $2100$ images of resolution $120 \times 160$. The first $770$ frames are outlier free. Here we use the first ``noisy'' $400$ frames as training data. The Alt Proj algorithm is used to obtain an initial estimate with rank, $r = 40$. The parameters used in all algorithms are exactly the same as in the MR and LB dataset. NORST achieves a ``test'' processing rate of $12$ frames-per-second.
\begin{figure}[ht!]
\begin{center}
\resizebox{.7\linewidth}{!}{
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\\    \newline
	\includegraphics[scale=.15]{figures/orig_SL460.jpg}
&
	\includegraphics[scale=.15]{figures/reprocs_pca_bg_SL60.jpg}
&
	\includegraphics[scale=.15]{figures/ncrpca_BG_SL460.jpg}
&
	\includegraphics[scale=.15]{figures/gd_BG_SL460.jpg}
&
	\includegraphics[scale=.15]{figures/grasta_BG_SL460.jpg}
&
	\includegraphics[scale=.15]{figures/rpca_BG_SL460.jpg}
\\    \newline
	\includegraphics[scale=.15]{figures/orig_SL600.jpg}
&
	\includegraphics[scale=.15]{figures/reprocs_pca_bg_SL200.jpg}
&
	\includegraphics[scale=.15]{figures/ncrpca_BG_SL600.jpg}
&
	\includegraphics[scale=.15]{figures/gd_BG_SL600.jpg}
&
	\includegraphics[scale=.15]{figures/grasta_BG_SL600.jpg}
&
	\includegraphics[scale=.15]{figures/rpca_BG_SL600.jpg}
\\    \newline
	\includegraphics[scale=.15]{figures/orig_SL1088.jpg}
&
	\includegraphics[scale=.15]{figures/reprocs_pca_bg_SL688.jpg}
&
	\includegraphics[scale=.15]{figures/ncrpca_BG_SL1088.jpg}
&
	\includegraphics[scale=.15]{figures/gd_BG_SL1088.jpg}
&
	\includegraphics[scale=.15]{figures/grasta_BG_SL1088.jpg}
&
	\includegraphics[scale=.15]{figures/rpca_BG_SL1088.jpg}
\\    \newline
	\subcaptionbox{original\label{1}}{\includegraphics[scale=.15]{figures/orig_SL1399.jpg}}
&
	\subcaptionbox{NORST\label{1}}{\includegraphics[scale=.15]{figures/reprocs_pca_bg_SL999.jpg}}
&
	\subcaptionbox{AltProj\label{1}}{\includegraphics[scale=.15]{figures/ncrpca_BG_SL1399.jpg}}
&
	\subcaptionbox{RPCA-GD\label{1}}{\includegraphics[scale=.15]{figures/gd_BG_SL1399.jpg}}
&
	\subcaptionbox{GRASTA\label{1}}{\includegraphics[scale=.15]{figures/grasta_BG_SL1399.jpg}}
&
	\subcaptionbox{PCP\label{1}}{\includegraphics[scale=.15]{figures/rpca_BG_SL1399.jpg}}
\end{tabular}
}
\caption{Comparison of visual performance in Foreground Background separation for the SwitchLight (SL) dataset. The recovered background images are shown at $t = t_\train +60, 200, 688, 999$. Note that because of the drastic change in environment, none of the techniques are able to detect the object properly.}
\end{center}
\end{figure} 

==> morost_icml_sims_main.tex <==
\Section{Empirical Evaluation}

\begin{figure}[t!]
\centering
\begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=1 by 1,
            %x descriptions at=edge bottom,
            y descriptions at=edge left,
        },
        % load the style created in the preamble
        my stylecompare,
        %ymin=1e-6, ymax=1e1,
        enlargelimits=false,
        width = .9\linewidth,
        height=3.7cm,
    ]
       \nextgroupplot[
            my legend style compare,
            ymode=log,
            %xlabel=$t$,
            xlabel={\small{$t$}},
            ylabel={\small{$\SE(\Phat_{(t)}, \P_{(t)})$}},
            %title=(a)
        ]
	        \addplot table[x index = {0}, y index = {1}]{\ltmodata};
	        \addplot table[x index = {0}, y index = {2}]{\ltmodata};
	        \addplot table[x index = {0}, y index = {3}]{\ltmodata};
	        \addplot table[x index = {0}, y index = {4}]{\ltmodata};
	        %\addplot table[x index = {0}, y index = {5}]{\ltmodata};
	        %\addplot table[x index = {0}, y index = {6}]{\ltmodata};
	        %\addplot table[x index = {0}, y index = {7}]{\ltmodata};
    \end{groupplot}
\end{tikzpicture}
%\vspace{-0.2in}
%\vspace{-0.25in}
\caption{\footnotesize{The plot of subspace error versus time for the online RST algorithms, plotted every $\alpha=300$ time instants. Time taken per sample (milliseconds) is shown in legend parentheses.
%Besides s-ReProCS, we also compare with the two popular RST heuristics from literature - ORPCA \cite{xu_nips2013_1} and GRASTA \cite{grass_undersampled}. %
}}
%\vspace{-0.2in}
\label{fig:Comparison}
\end{figure}



%All time comparisons are performed on a Desktop Computer with Intel$^{\textsuperscript{\textregistered}}$ Xeon E$3$-$1240$ $8$-core CPU @ $3.50$GHz and $32$GB RAM.
\subsubsection{Synthetic Data}
We generated the subspaces using $\P_j = e^{\tilde\delta_j \bm{B}_j} \P_{j-1}$ (as done in \cite{grass_undersampled}) where $\tilde\delta_j$ controls the subspace change and $\bm{B}_j$'s are skew-symmetric matrices. In our experiments we use $n = 1000$, $d = 12000$, $r=30$, $J = 2$, $t_1 = 3000$, $t_2 = 8000$, $r = 30$, $\tilde\delta_1 = \tilde\delta_2 = 0.001$. $\P_0$ is generated by ortho-normalizing columns of an $n \times r$ i.i.d standard normal matrix. The subspace coefficients $\at \in \mathbb{R}^{r}$ are generated as independent zero-mean, bounded (uniform) random variables with condition number of their covariance $f = 50$. We generated the support $\T_t$ of sparse outliers using the Moving Object Model of \cite{rrpcp_dynrpca}. We used the first $t_{\train} = 3.3 r = 100$ frames as the training data with fewer outliers: for this period we used $b_0 = 0.01$, and for $t > t_\train$, we used $s/n = 0.05$ and $b_0 = 0.3$. The non-zero magnitudes of $\xt$ are generated as i.i.d as $uniform[10, 20]$. The algorithm parameters are set as in Algorithm \ref{algo:auto-reprocs-pca}, $K=8$, $\alpha=300$. %We run all batch algorithms on sub-matrices $\Y_{(t_\train, k \alpha]}$ $k \in [1, (\tmax - t_\train)/\alpha])$.
As shown in Fig. \ref{fig:Comparison}, NORST is significantly better than all the RST methods - s-ReProCS, and two popular heuristics from literature - ORPCA \cite{xu_nips2013_1} and GRASTA \cite{grass_undersampled}.

We provide a separate comparison of offline techniques in Table 2. As can be seen, offline NORST outperforms all static RPCA methods, both for the moving object outlier support model and for the commonly used random Bernoulli support model. All results are averaged over $10$ independent runs. Complete details in Appendix \ref{sims_detail}.%owing to large $\outfracrow$. It is also faster than all techniques except GRASTA.

\begin{table}[h!]
\begin{center}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{cccc} \toprule
Outlier Model & RPCA-GD & AltProj & \bf{Offline-NORST} \\
& ($92.2$ms) & ($70.8$ms) & ($\bm{1.7}$\bf{ms}) \\ \toprule
Mov. Obj. & $4.283$ & $4.363$ & $\bm{3.5 \times 10^{-4}}$ \\
Bernoulli & $0.158$& $0.269$ & $\bm{3.4 \times 10^{-4}}$ \\ \bottomrule
\end{tabular}
}
\end{center}
%\vspace{-.17in}
\label{tab:offline}
\caption{\footnotesize{Comparison of $\|\Lhat - \L\|_F/\|\L\|_F$ for offline RPCA methods including offline NORST. Average time given in parentheses.}}
%\vspace{-.1in}
\end{table}


\subsubsection{Video}
%\input{video_main_icml}
We also evaluated NORST for the background-subtraction task. Sample results are presented in Figure \ref{fig:video_res}. The NORST parameters are set as $\alpha = 60$, $K=3$, $r = 40$ and $\xi_t = \|\bpsi \lhat_{t-1}\|$. Complete details in Appendix \ref{sims_detail}.%






==> video_main_icml.tex <==
\begin{figure*}[ht!]
%\vspace{-0.2in}
\centering
\resizebox{.9\linewidth}{!}{
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\tiny{Video Frame} & \tiny{\bf{NORST} ($\bm{16.5}$\bf{ms})} & \tiny{AltProj($26.0$ms)} & \tiny{RPCA-GD($29.5$ms)} & \tiny{GRASTA} ($2.5$ms)& \tiny{PCP} ($44.6$ms) %\vspace{-.11cm}
\\
	\includegraphics[scale=0.19, trim={2.1cm, 0cm, 2.1cm, 0.5cm}, clip]{figures/orig_MR1030.jpg}
&
	\includegraphics[scale=0.178, trim={2.1cm, 0cm, 2.1cm, 0.5cm}, clip]{figures/reprocs_pca_bg_curtain_theory630.jpg}
&
	\includegraphics[scale=0.178, trim={2.1cm, 0cm, 2cm, 0.5cm}, clip]{figures/ncrpca_BG_MR1030.jpg}
&
	\includegraphics[scale=0.191, trim={2.5cm, 0cm, 2.1cm, 0.5cm}, clip]{figures/gd_BG_MR1030.jpg}
&
	\includegraphics[scale=0.18, trim={2.1cm, 0cm, 2.1cm, 0.5cm}, clip]{figures/grasta_BG_MR1030.jpg}
&
	\includegraphics[scale=0.18, trim={2.1cm, 0cm, 2.1cm, 0.5cm}, clip]{figures/rpca_BG_MR1030.jpg}
%&
%	\includegraphics[scale=0.191, trim={2.1cm, 0cm, 2.1cm, 0.5cm}, clip]{figures/stream_BG_MR540.jpg}
\\    \newline
\tiny{Video Frame} & \tiny{\bf{NORST} ($\bm{85.4}$\bf{ms})} & \tiny{AltProj($95.7$ms)} & \tiny{RPCA-GD($122.5$ms)} & \tiny{GRASTA} ($22.6$ms) & \tiny{PCP} ($318.3$ms)  \\

		\includegraphics[scale=.128, trim={2cm, 0cm, 2cm, 0cm}, clip]{figures/orig_SL1399.jpg}
&
	\includegraphics[scale=.128, trim={1.7cm, 0cm, 1.7cm, 0cm}, clip]{figures/reprocs_pca_bg_SL999.jpg}
&
	\includegraphics[scale=.135, trim={1.7cm, 0cm, 1.7cm, 0cm}, clip]{figures/ncrpca_BG_SL1399.jpg}
&
	\includegraphics[scale=.13, trim={2cm, 0cm, 2cm, 0cm}, clip]{figures/gd_BG_SL1399.jpg}
&
	\includegraphics[scale=.125, trim={1cm, 0cm, 1cm, 0cm}, clip]{figures/grasta_BG_SL1399.jpg}
&
	\includegraphics[scale=.13, trim={2cm, 0cm, 2cm, 0cm}, clip]{figures/rpca_BG_SL1399.jpg}
%\\    \newline
%%\vspace{-.1cm}
%\tiny{Video Frame} & \tiny{\bf{NORST} ($\bm{72.5}$\bf{ms})} & \tiny{AltProj($133.1$ms)} & \tiny{RPCA-GD($113.6$ms)} & \tiny{GRASTA} ($18.9$ms) & \tiny{PCP} ($240.7$ms)\\
%
%	\includegraphics[scale=0.13, trim={2cm, 0cm, 2cm, 0cm}, clip]{figures/orig_LB1010.jpg}
%&
%	\includegraphics[scale=0.13, trim={2cm, 0cm, 2cm, 0cm}, clip]{figures/reprocs_pca_bg_LB610.jpg}
%&
%	\includegraphics[scale=0.137, trim={2cm, 0cm, 2cm, 0cm}, clip]{figures/ncrpca_BG_LB1010.jpg}
%&
%	\includegraphics[scale=0.137, trim={2cm, 0cm, 2cm, 0cm}, clip]{figures/gd_BG_LB1010.jpg}
%&
%	\includegraphics[scale=0.137, trim={2cm, 0cm, 2cm, 0cm}, clip]{figures/grasta_BG_LB1010.jpg}
%&
%	\includegraphics[scale=0.125, trim={1cm, 0cm, 1cm, 0cm}, clip]{figures/rpca_BG_LB1010.jpg}
\end{tabular}
}
%\vspace{-0.15in}
%\caption{\small{Background recovery. For \texttt{MR} and \texttt{SL} sequences (first two rows), only NORST, s-ReProCS does not contain the person or even his shadow. NORST is faster than all except GRASTA. For \texttt{LB} NORST is as good as PCP, GRASTA, and s-ReProCS while others fail. Time taken per frame is shown in parentheses.%
%}}
\caption{\small{Background Recovery. NORST is the only technique that works for both sequences. All the other algorithms exhibit some artifacts. Row 2: only NORST does not contain the person or even his shadow. NORST is faster than all except GRASTA (which does not work). In fact, the GRASTA output slightly lags the actual frame, and hence, it appears that the person is sitting. Time taken per frame is shown in parentheses.}}
\label{fig:video_res}
%\vspace{-0.15in}
\end{figure*} 
